Towards Spatio-Temporal Aware Traffic Time Series Forecasting--Full Version

Traffic time series forecasting is challenging due to complex spatio-temporal dynamics time series from different locations often have distinct patterns; and for the same time series, patterns may vary across time, where, for example, there exist certain periods across a day showing stronger temporal correlations. Although recent forecasting models, in particular deep learning based models, show promising results, they suffer from being spatio-temporal agnostic. Such spatio-temporal agnostic models employ a shared parameter space irrespective of the time series locations and the time periods and they assume that the temporal patterns are similar across locations and do not evolve across time, which may not always hold, thus leading to sub-optimal results. In this work, we propose a framework that aims at turning spatio-temporal agnostic models to spatio-temporal aware models. To do so, we encode time series from different locations into stochastic variables, from which we generate location-specific and time-varying model parameters to better capture the spatio-temporal dynamics. We show how to integrate the framework with canonical attentions to enable spatio-temporal aware attentions. Next, to compensate for the additional overhead introduced by the spatio-temporal aware model parameter generation process, we propose a novel window attention scheme, which helps reduce the complexity from quadratic to linear, making spatio-temporal aware attentions also have competitive efficiency. We show strong empirical evidence on four traffic time series datasets, where the proposed spatio-temporal aware attentions outperform state-of-the-art methods in term of accuracy and efficiency. This is an extended version of "Towards Spatio-Temporal Aware Traffic Time Series Forecasting", to appear in ICDE 2022 [1], including additional experimental results.

==> results/dataset.tex <==
\begin{table}[h]
\centering
\begin{tabular}{|ccc|} 
\toprule
Dataset        & Number of sensors $N$ & Time range                       \\ 
\hline
\textbf{PEMS03} & 358               & 9/1/2018 - 11/30/2018                     \\
\textbf{PEMS04} & 307               & 1/1/2018 - 2/28/2018                      \\
\textbf{PEMS07} & 883               & 5/1/2017 - 8/31/2017                      \\
\textbf{PEMS08} & 170               & 7/1/2016 - 8/31/2016                      \\
\bottomrule
\end{tabular}
\caption{Dataset description}
\label{table:dataset}
\vspace{-5pt}
\end{table}


==> revision_files/astgnn.tex <==
\begin{table}[h]
\centering

\begin{tabular}{|c|c|c|c|} 
\hline
\multicolumn{2}{|c|}{Baseline methods}                                                                                                          & ST-agnostic       & ST-aware          \\ 
\hline
Dataset                                                                           & Metric                                                      & $\texttt{ASTGNN}$ & $\texttt{ST-WA}$  \\ 
\hline
\multirow{4}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{PEMS03}\\N=358\\\end{tabular}} & MAE                                                         & \textbf{15.07}    & 15.17             \\
                                                                                  & MAPE                                                        & \textbf{15.80}    & 15.83             \\
                                                                                  & RMSE                                                        & 26.88             & \textbf{26.63}    \\
                                                                                  & \begin{tabular}[c]{@{}c@{}}Training\\(s/epoch)\end{tabular} & 142.69            & \textbf{56.85}    \\ 
\hline
\multirow{4}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{PEMS04}\\N=307\\\end{tabular}} & MAE                                                         & 19.26             & \textbf{19.06 }   \\
                                                                                  & MAPE                                                        & 31.16             & \textbf{12.52}    \\
                                                                                  & RMSE                                                        & 31.16             & \textbf{31.02}    \\
                                                                                  & \begin{tabular}[c]{@{}c@{}}Training\\(s/epoch)\end{tabular} & 103.82            & \textbf{21.93}    \\ 
\hline
\multirow{4}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{PEMS07}\\N=883\\\end{tabular}} & MAE                                                         & 22.23             & \textbf{20.74 }   \\
                                                                                  & MAPE                                                        & 9.25              & \textbf{8.77}     \\
                                                                                  & RMSE                                                        & 35.95             & \textbf{34.05}    \\
                                                                                  & \begin{tabular}[c]{@{}c@{}}Training\\(s/epoch)\end{tabular} & 1661.32           & \textbf{242.81}   \\ 
\hline
\multirow{4}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{PEMS08}\\N=170\\\end{tabular}} & MAE                                                         & 15.98             & \textbf{15.41}    \\
                                                                                  & MAPE                                                        & 9.97              & \textbf{9.94}     \\
                                                                                  & RMSE                                                        & 25.67             & \textbf{24.62}    \\
                                                                                  & \begin{tabular}[c]{@{}c@{}}Training\\(s/epoch)\end{tabular} & 59.41             & \textbf{17.78}    \\
\hline
\end{tabular}
\caption{Comparison with \texttt{ASTGNN}, $H=12$, $U=12$ }
\label{table:results_astgnn}
\end{table}
% \BY{place the number of sensors under each data set so the reviewer can see it w.r.t. the scalability of sensor numbers}

==> revision_files/long_range.tex <==
\begin{table*}[h]
% \renewcommand{\tabcolsep}{2.2pt}
\centering
\begin{tabular}{|c|cccc|cccc|cccc|} 
\hline
\multirow{2}{*}{}                                            & \multicolumn{4}{c|}{$H=12$}                                            & \multicolumn{4}{c|}{$H=36$}                                            & \multicolumn{4}{c|}{$H=120$}                                                     \\
                                                             & $\texttt{Trans}$ & $\texttt{LogS}$ & $\texttt{Ref}$ & $\texttt{ST-WA}$ & $\texttt{Trans}$ & $\texttt{LogS}$ & $\texttt{Ref}$ & $\texttt{ST-WA}$ & $\texttt{Trans}$     & $\texttt{LogS}$      & $\texttt{Ref}$ & $\texttt{ST-WA}$  \\ 
\hline
MAE                                                          & 31.28            & 27.88           & 27.25          & \textbf{19.06}   & 30.25            & 29.19           & 26.85          & \textbf{18.90 }  & \multirow{4}{*}{OOM} & \multirow{4}{*}{OOM} & 24.78          & \textbf{18.90 }   \\
MAPE                                                         & 34.23            & 28.55           & 28.00          & \textbf{12.52}   & 32.66            & 31.08           & 29.25          & \textbf{12.43 }  &                      &                      & 24.75          & \textbf{12.92 }   \\
RMSE                                                         & 43.85            & 40.72           & 40.21          & \textbf{31.02}   & 42.83            & 41.56           & 38.95          & \textbf{30.92 }  &                      &                      & 35.65          & \textbf{30.69 }   \\
\begin{tabular}[c]{@{}c@{}}Training \\(s/epoch)\end{tabular} & 27.58            & 26.21           & 22.62          & \textbf{21.93 }  & 128.82           & 120.17          & 67.37          & \textbf{64.65 }  &                      &                      & 263.54         & \textbf{145.18 }  \\
\hline
\end{tabular}

\caption{Impact of window size $H$,  \textbf{PEMS04}.}
\label{table:long_range_res}
\end{table*}
%  \BY{remove WA-SCA}


% \begin{table}
% \centering
% \caption{Impact of window size $H$ on \textbf{PEMS04}.}
% \label{table:long_range}
% \begin{tabular}{|c|ccccc|ccccc|ccccc|} 
% \hline
% \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\\~\\\end{tabular}} & \multicolumn{5}{c|}{$H=12$}                                                                & \multicolumn{5}{c|}{$H=36$}                                                                & \multicolumn{5}{c|}{$H=120$}                                                                         \\
%                                                               & $\texttt{Trans}$ & $\texttt{LogS}$ & $\texttt{Ref}$ & $\texttt{WA-SCA}$ & $\texttt{ST-WA}$ & $\texttt{Trans}$ & $\texttt{LogS}$ & $\texttt{Ref}$ & $\texttt{WA-SCA}$ & $\texttt{ST-WA}$ & $\texttt{Trans}$     & $\texttt{LogS}$      & $\texttt{Ref}$ & $\texttt{WA-SCA}$ & $\texttt{ST-WA}$  \\ 
% \hline
% MAE                                                            & 31.28            & 27.88           & 27.25          & 23.92             & \textbf{19.06}   & 30.25            & 29.19           & 26.85          & 21.88             & 18.90            & \multirow{5}{*}{OOM} & \multirow{5}{*}{OOM} & 24.78          & 20.67             & 18.90             \\
% MAPE                                                           & 34.23            & 28.55           & 28.00          & 15.91             & \textbf{12.52}   & 32.66            & 31.08           & 29.25          & 14.13             & 12.43            &                      &                      & 24.75          & 14.05             & 12.92             \\
% RMSE                                                           & 43.85            & 40.72           & 40.21          & 37.41             & \textbf{31.02}   & 42.83            & 41.56           & 38.95          & 34.83             & 30.92            &                      &                      & 35.65          & 32.93             & 30.69             \\
% Training                                                       & 27.58            & 26.21           & 22.62          & 5.81              & \textbf{21.93}   & 128.82           & 120.17          & 67.37          & 16.93             & 64.65            &                      &                      & 263.54         & 34.55             & 145.18            \\
% Mem Usage                                                      & 3.20             & 3.00            & 2.71           & 1.66              & 8.14             & 19.32            & 18.25           & 5.43           & 2.42              & 10.26            &                      &                      & 19.26          & 3.85              & 10.25             \\
% \hline
% \end{tabular}
% \end{table}

==> revision_files/longformer.tex <==


\begin{table}[h]
\centering

\begin{tabular}{|c|c|c|c|} 
\hline
\multicolumn{2}{|c|}{Baseline methods                                                                                                          }  & ST-agnostic           & ST-aware            \\ 
\hline
Dataset                                                                            & Metric                                                       & $\texttt{LongFormer}$ & $\texttt{ST-WA}$    \\ 
\hline
\multirow{4}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{PEMS03}\\N=358\\\end{tabular}}  & MAE                                                          & 17.50                 & \textbf{15.17 }     \\
                                                                                   & MAPE                                                         & 16.80                 & \textbf{15.83 }     \\
                                                                                   & RMSE                                                         & 30.24                 & \textbf{26.63}      \\
                                                                                   & \begin{tabular}[c]{@{}c@{}}Training\\(s/epoch)\end{tabular}  & 137.83                & \textbf{56.85}      \\ 
\hline
\multirow{4}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{PEMS04}\\N=307\\\end{tabular}}  & MAE                                                          & 23.83                 & \textbf{19.06}      \\
                                                                                   & MAPE                                                         & 15.57                 & \textbf{12.52}      \\
                                                                                   & RMSE                                                         & 37.19                 & \textbf{31.02}      \\
                                                                                   & \begin{tabular}[c]{@{}c@{}}Training\\(s/epoch)\end{tabular}  & 68.40                 & \textbf{21.93}      \\ 
\hline
\multirow{4}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{PEMS07}\\N=883\\\end{tabular}}  & MAE                                                          & 26.80                 & \textbf{20.74}      \\
                                                                                   & MAPE                                                         & 12.11                 & \textbf{8.77}       \\
                                                                                   & RMSE                                                         & 42.95                 & \textbf{34.05}      \\
                                                                                   & \begin{tabular}[c]{@{}c@{}}Training\\(s/epoch)\end{tabular}  & 608.43                & \textbf{242.81}     \\ 
\hline
\multirow{4}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{PEMS08}\\N=170\\\end{tabular}}  & MAE                                                          & 18.52                 & \textbf{15.41}      \\
                                                                                   & MAPE                                                         & 13.66                 & \textbf{9.94}       \\
                                                                                   & RMSE                                                         & 28.68                 & \textbf{24.62}      \\
                                                                                   & \begin{tabular}[c]{@{}c@{}}Training\\(s/epoch)\end{tabular}  & 32.61                 & \textbf{17.78}      \\
\hline
\end{tabular}
\caption{Comparison with \texttt{LongFormer}, $H=12$, $U=12$ }
\label{table:results_longformer}
\end{table}

==> revision_files/naive.tex <==
\begin{table*}[h]
\centering
\renewcommand{\tabcolsep}{4pt}


\begin{tabular}{|c|c|c|c|c|c|} 
\hline
\begin{tabular}[c]{@{}c@{}}\\Dataset\end{tabular} & Metric                                                      & $\texttt{HWES}$ & $\texttt{Transformer}$ & $\texttt{W-ATT}$ & $\texttt{ST-WA}$         \\ 
\hline
\multirow{4}{*}{\textbf{PEMS03}}                  & MAE                                                         & 23.77           & 22.49                  & 17.87            & \textbf{15.17}           \\
                                                  & MAPE                                                        & 22.01           & 21.95                  & 17.00            & \textbf{15.83}           \\
                                                  & RMSE                                                        & 38.28           & 37.45                  & 29.86            & \textbf{\textbf{26.63}}  \\
                                                  & \begin{tabular}[c]{@{}c@{}}Runtime \\(seconds)\end{tabular} & 3297            & 13332                  & \textbf{2050 }   & 11370                    \\ 
\hline
\multirow{4}{*}{\textbf{PEMS04}}                  & MAE                                                         & 32.06           & 29.69                  & 23.09            & \textbf{\textbf{19.06}}  \\
                                                  & MAPE                                                        & 22.84           & 20.71                  & 15.57            & \textbf{\textbf{12.52}}  \\
                                                  & RMSE                                                        & 47.71           & 45.43                  & 36.61            & \textbf{\textbf{31.02}}  \\
                                                  & \begin{tabular}[c]{@{}c@{}}Runtime \\(seconds)\end{tabular} & 2827            & 5040                   & \textbf{1170 }   & 4386                     \\ 
\hline
\multirow{4}{*}{\textbf{PEMS07}}                  & MAE                                                         & 33.56           & 30.96                  & 24.47            & \textbf{\textbf{20.74}}  \\
                                                  & MAPE                                                        & 17.32           & 14.35                  & 10.72            & \textbf{\textbf{8.77}}   \\
                                                  & RMSE                                                        & 55.47           & 48.52                  & 39.55            & \textbf{\textbf{34.05}}  \\
                                                  & \begin{tabular}[c]{@{}c@{}}Runtime \\(seconds)\end{tabular} & 8132            & 37652                  & \textbf{5760 }   & 48562                    \\ 
\hline
\multirow{4}{*}{\textbf{PEMS08}}                  & MAE                                                         & 28.29           & 25.42                  & 17.76            & \textbf{\textbf{15.41}}  \\
                                                  & MAPE                                                        & 18.76           & 16.53                  & 11.85            & \textbf{\textbf{9.94}}   \\
                                                  & RMSE                                                        & 42.12           & 38.58                  & 28.83            & \textbf{\textbf{24.62}}  \\
                                                  & \begin{tabular}[c]{@{}c@{}}Runtime \\(seconds)\end{tabular} & 1565            & 9122                   & \textbf{916 }    & 3556                     \\
\hline
\end{tabular}

\caption{Overall Accuracy of Enhanced versions of \texttt{ATT}, $H=12$, $U=12$}
\label{table:naive}
\end{table*}

==> revision_files/recurrent_connection_results.tex <==
\begin{table*}[h]
\centering
% \renewcommand{\tabcolsep}{1pt}

\begin{tabular}{|c|cc|cc|cc|} 
\hline
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\\~\\~\\\end{tabular}} & \multicolumn{2}{c|}{$H=12$}           & \multicolumn{2}{c|}{$H=36$}           & \multicolumn{2}{c|}{$H=120$}           \\
                                                                  & $\texttt{ST-WA-R}$ & $\texttt{ST-WA}$ & $\texttt{ST-WA-R}$ & $\texttt{ST-WA}$ & $\texttt{ST-WA-R}$ & $\texttt{ST-WA}$  \\ 
\hline
MAE                                                               & 19.49              & \textbf{19.06}  & 19.40              & \textbf{18.90}  & 19.19              & \textbf{18.90}   \\
MAPE                                                              & 12.90              & \textbf{12.52}  & 12.79              & \textbf{12.43}  & 12.76              & \textbf{12.92}    \\
RMSE                                                              & 31.09              & \textbf{31.02}  & 30.93              & \textbf{30.92}  & 30.74              & \textbf{30.69}   \\
\begin{tabular}[c]{@{}c@{}}Training \\(s/epoch)\end{tabular}      & \textbf{21.54}    & 21.93            & \textbf{63.85 }    & 64.65            & \textbf{142.44}   & 145.18            \\
\hline
\end{tabular}

\caption{Impact of recurrent connections, \textbf{PEMS04}.}
\label{table:recurrent_connection}
\end{table*}

==> revision_files/reviewer1.tex <==
\section{Reviewer \#1}
\setlength{\parindent}{0em}

\textbf{R1O1}: In Equation 13, why the output of MLP of a single hidden state could measure the importance of its input? Please give an intuitive explanation here.

\textbf{Response}: The MLP takes as input all $p$ proxies’ hidden representations, but not a single proxy’s hidden representation. In Equation 12, $\textbf{h}_w^{(i)}$ represents all $p$ proxies in the window $w$ for sensor $i$. In other words, $\textbf{h}_w^{(i)}=\left\{\textbf{h}_{w,j}^{(i)}\right\}
_{j=1}^{p}$. In the running example shown in Figure 6 and Figure 7 in the revised paper, we have $p=2$ proxies per window. Thus, in Figure 7 in the revised paper, we use two blue rectangles for $\textbf{h}_w^{(i)}$, indicating the $p=2$ proxies' hidden representations, which are fed into the weighting network as the input. The output of the weighting network $\textbf{A}_w^{(i)}$ also has two rectangles representing the corresponding weights of the $p=2$ proxies. Then, we compute the weighted proxies, which are finally summed into a single, aggregated representation $\hat{\textbf{h}}_w^{(i)}$, shown as a single rectangle in the end.

We updated Figure 7 in the revised paper, to make it more explicit that the weights are computed for all $p$ proxies.

\vspace{2em}
\textbf{R1O2}:  The paper first states that $\textbf{P} \in R^{W*N*p*d}$ is a learnable parameter, to my understanding, this implies that $\textbf{P}_w^{(i)} \in R^{p*d}$ for $w \in [W], i \in [N]$ are embeddings learned from randomly initialization but Equation 14 states that $\textbf{P}_w^{(i)}$ is computed from $\textbf{P}_{w-1}^{(i)}$, which are inconsistent and contradicted. Please clarify how $\textbf{P}_w^{(i)}$ is computed. In addition, even if $\textbf{P}_w^{(i)}$ is computed from $\textbf{P}_{w-1}^{(i)}$, the hidden state in Equation 14 should be $\hat{\textbf{h}}_{w-1}^{(i)}$ instead of $\hat{\textbf{h}}_{w}^{(i)}$ because $\hat{\textbf{h}}_{w}^{(i)}$ itself depends on $\textbf{P}_w^{(i)}$; moreover, this also means you have to calculate $\textbf{P}_w^{(i)}$ sequentially along the window dimension that would incur additional computational overhead in comparison to the canonical self-attention mechanism, in particular, when the sequence is very long and window sizes are large this would become a serious bottleneck and the reviewer doubts if such design could really bring speed advantage. Correct me if I am wrong.

\textbf{Response}: It is true that $\textbf{P}_w^{(i)}$ are embeddings learned from random initialization. Yes, there are errors in Equation 14, where $\hat{\textbf{h}}_{w}^{(i)}$ should be $\hat{\textbf{h}}_{w-1}^{(i)}$ as the reviewer identified; and $\textbf{P}_{w-1, j}^{(i)}$ should be $\textbf{P}_{w, j}^{(i)}$. This means that a randomly initialized $\textbf{P}_w^{(i)}$ is fused with the hidden state $\hat{\textbf{h}}_{w-1}^{(i)}$ from the previous window. This indeed makes the computation sequential. The updated Equation 14 is shown below, which is also updated in the revision. 

%\begin{equation}\label{eq:recurrent}
  $$  \textbf{P}_{w,j}^{(i)} = \vartheta(\hat{\textbf{h}}^{(i)}_{w-1} \; || \; \textbf{P}^{(i)}_{w, j}) \; \; \; \forall \; j \in [1, p].
$$%\end{equation}

\input{revision_files/recurrent_connection_results}

\input{revision_files/long_range}

\hspace{0.4cm} Next, to evaluate the impact of the recurrent connection that fuses with the previous hidden state $\hat{\textbf{h}}_{w-1}^{(i)}$, we have performed an additional ablation study where we consider a variant $\texttt{ST-WA-R}$ that  removes the recurrent connection. Table \ref{table:recurrent_connection}  in the revision report, shows the results. We can see that when the recurrent connections are removed, the accuracy decreases which highlights its importance. For training time  (seconds/epoch), as the input sequence $H$ increases, the runtime increases for both models. However, the recurrent connections in \texttt{ST-WA} incur negligible runtime overhead when comparing to \texttt{ST-WA-R}. The recurrent connections offer a trade-off when accuracy is more important then efficiency. 




\vspace{2em}
\textbf{R1O3}: The paper states that it stacks multiple layers of attention. The reviewer is wondering if all layers use the same learnable parameter $P \in R^{W*N*p*d}$. It does not make sense to me that all layers adopt the same $P$ because the sequence is shrunk as the depth grows.

\textbf{Response}: Each window attention layer has its own set of learnable parameters. This is consistent with existing models using multiple layers of canonical self-attentions, e.g., Transformers, where different self-attention layers have its own set of projection
matrices (cf. Section III-B). We have revised the paper and added a sentence in Section VI.D to highlight that each layer has its own set of proxies $\textbf{P}$. 


\vspace{2em}
\textbf{R1O4}: Moreover, many strategies have already been proposed in the literature to reduce the sequence length square complexity of self-attention such as [1, 2] and they have been widely used in the community. Is there any necessary to propose a new one and what are the advantages of the proposed one compared with them? In the experiments, the length of the longest sequences seems to be 120. From the reviewer's experience, the canonical self-attention could handle such a magnitude of lengths very well. The motivation of the proposed attention layer is further weakened. Could the author provide the training times (the models with both the canonical self-attention and the proposed one) varying against sequence lengths?


[1] Reformer: The Efficient Transformer, ICLR 2021.

[2] Enhancing the Locality and Breaking the Memory Bottleneck of Transformer on Time Series Forecasting, NeurIPS 2019.

\textbf{Response}: First, we would like to highlight that the complexity of \texttt{Reformer} [1] and \texttt{LogSparse} [2] are  $\mathcal{O}(H \; lgH)$ and $O(H \; (lgH)^2)$, whereas our proposal has only  $\mathcal{O}(H)$. We do need such an efficient attention to ensure the overall efficiency, as the spatio-temporal aware modeling incurs additional overhead. It is true that canonical self-attention can handle sequences bigger than 120, but our setup is slightly different as we process $N$ different time-series corresponding to $N$ different locations at the same time. In the original setup of canonical self-attention only $H^2$ attention scores needs to be computed, while in our setup we need to compute $N \times H^2$ which have a big impact on the memory usage. 



\hspace{0.4cm} To evaluate the accuracy and training time of the relevant methods, we performed an additional experiment in which we compare the following methods suggested by the reviewer: (1) Transformer using canonical self-attentions (\texttt{Trans}), (2) \texttt{LogSparse} (\texttt{LogS}), (3) \texttt{Reformer} (\texttt{Ref}), and (4) the proposed \texttt{ST-WA}. The results are shown in Table \ref{table:long_range_res}  in the revision report. The results show that our proposal outperforms the other three methods in terms of both accuracy and efficiency. We would like to note that \texttt{Trans} is slightly different from \texttt{SA},  which we mentioned in the author feedback phase---\texttt{Trans} does not model entity correlations whereas \texttt{SA} (cf. Table VIII in the revised paper) does. %for a fair comparison with \texttt{LogS} and \texttt{Ref}. 


%First we explore the temporal modeling capabilities of \texttt{Trans}, \texttt{LogS}, \texttt{Ref}, as they can not directly support entity correlation modeling, when to our \textttt{WA-SCA}. Table \ref{table:long_range_res} shows the results. We can observe that \texttt{Trans} achieves the worst performance, while being the slowest. Next we can observe that \texttt{LogS} achieves better accuracy while being more efficient, which aligns with the complexity analysis. Furthermore we observe that \texttt{Ref} outperforms \texttt{Trans} and \texttt{LogS} in terms of accuracy and efficiency. Next, we can observe that our proposal \textttt{WA-SCA} significantly outperforms other baselines in terms of accuracy and efficiency which makes spatio-temporal aware modeling possible. Finally, we can observe that the final model \texttt{ST-WA} which is spatio-temporal aware and explicitly models entity correlation achieves significantly better results while still being the fastest when compared with the other baselines which justifies our design choices.    






\vspace{2em}
\textbf{R1O5}: The newly developed traffic forecasting model [3] is missed from the paper. It should be added to Table II and experiments.

[3] Learning Dynamics and Heterogeneity of Spatial-Temporal Graph Data for Traffic Forecasting, TKDE 2021.

\textbf{Response}: We have added the newly developed traffic forecasting model \texttt{ASTGNN} [3] into Table II in the revised paper. \texttt{ASTGNN} belongs to Spatial-Temporal agnostic methods, as it is based on attentions which share the same projection matrices across all sensors and across different time periods. 

We also report its performance in Table IV in the revised paper. We note that the results of some baselines such as \texttt{Graph WaveNet} and \texttt{STGCN} in the \texttt{ASTGNN} paper are inconsistent with the results of other recent papers such as \cite{agcrn} and our paper. For a fair comparison, we have
used the original implementation of \texttt{ASTGNN} and test it under our setup. From Table \ref{table:results_astgnn} in the revision report, we observe that our proposal outperforms \texttt{ASTGNN} in terms of accuracy on 10 out of 12 metrics over four data sets. Furthermore, we observe that \texttt{ASTGNN} is significantly slower that \texttt{ST-WA} and it does not scale well w.r.t. the number of sensors. If we look at the runtime for \texttt{PEMS07}, which has the most number of sensors, we can observe that \texttt{ST-WA} is more than 5 times faster. 



\input{revision_files/astgnn}


==> revision_files/reviewer2.tex <==
\section{Reviewer \#2}

\textbf{R2O1}: The motivation for this work could be improved. According to the authors' description, I guess authors were inspired by dynamic networks (i.e., CondConv.) and want to find an efficient solution to realize dynamics as well as maintain efficiency. Not like the straightforward method that employs a distinct set of projection matrices for each sensor, they reduce the memory consumption by decomposing the matrix into two small matrices and sharing one of them. Concretely, they introduce a VAE-typed architecture to decompose matrix. However, the author did not explain why introducing VAE rather than directly decomposing the matrix. Besides, there should be more convincing reasons for assuming the Gaussian distribution, rather than a re-parameterization capability.

\textbf{Response}: We agree that our work has been partially inspired by dynamic networks i.e., CondConv, as we already cite this work in the Related Work section, and that we aim for an efficient way of achieving similar behaviour. We opt for a variational encoder to generate model parameters due to its ability to capture the distributions of the input data, which better generalize to cases that were not seen during training. A deterministic variant, i.e, directly decomposing the matrix as suggested by the reviewer, fails to do so. Empirical evidence in Table XI in the revised paper shows that our proposal outperforms its deterministic variant. 

Since we do not rely on any prior knowledge of the distributions of the hidden factors, and since many real world processes follow Gaussian distributions~\cite{anderson1962introduction}, we assume they follow Gaussian distributions. Furthermore, this assumption is well used and accepted in stochastic models such as \cite{kingma2013auto,gaussian1,gaussian2,gaussian3}. We have modified the paper (cf. Section IV-A) to further clarify this design choice. 




\vspace{2em}
\textbf{R2O2}: The authors evade mention similar methods, i.e., lacking the reference of VAE and sliding window attention. They should add some details when comparing their method to recent sliding window attention.

\textbf{Response}: We added references to \texttt{VAE} in Section IV.A. 


\hspace{0.4cm} We also added a detailed review of sliding window attention methods in Section II. In sliding window attentions, e.g., Longformer \cite{beltagy2020longformer}, each timestamp considers a sliding window of length $S$, covering its past and future neighboring timestamps. As such each timestamp attends only to the $S$ timestamps in the sliding window. This leads to $\mathcal{O}(HS)$ complexity, where $H$ is the length of time series. In contrast, we do not use sliding windows but split a time series into $H/S$ static windows. In each window, we introduce a small constant number of  learnable proxies to replace the Query and compute attention scores between each timestamp and the proxies, resulting in $\mathcal{O}(H)$ complexity, which is more efficient. Furthermore, the output size of the sliding window attention is the same as the input size $H$, whereas the output size of the proposed window attention is $H/S$. The reduced output sizes make multi-layer attention structures more efficient as the computations in later layers keep reducing.

\input{revision_files/longformer}
\input{revision_files/naive}


\hspace{0.4cm} Furthermore, as suggested, we added a recent and popular sliding window attention based method $\texttt{LongFormer}$ \cite{beltagy2020longformer} as a baseline to the main experiments. The results can be seen in Table \ref{table:results_longformer} in the revision report. We observe that our proposal significantly outperforms $\texttt{LongFormer}$ in terms of accuracy and efficiency on all datasets.  





\vspace{2em}
\textbf{R2O3}: There seems to be a bit of a controversy surrounding the network design: the use of the dynamic mechanism to increase the model's capability but decrease efficiency, and replacing global self-attention with local ones to obtain efficiencies but sacrificing the performance.


\textbf{Response}: We would like to clarify the design choices. We acknowledge that the ST-Aware modeling improves model capability but incurs additional computation overhead. To compensate for this and ensure overall efficiency, we propose a more efficient window attention with linear complexity. However, the window attention does not sacrifice accuracy because (1) the learnable proxies are more capable of capturing information within windows than self-attentions, (2) the recurrent connections ensure the temporal receptive field is not broken, and (3) the skip connections in different layers allow for multiple gradient shortcuts.

\hspace{0.4cm} Table VIII in the revised paper, provides empirical evidence where the proposed Window Attention is not only fast but also more accurate than canonical self-attention. In addition, from Figure 9 in the revised paper, we observe that even with the additional overhead introduced by the ST-aware modeling, our proposal is the fastest, especially when the input length increases. We have modified the introduction (cf. Section I) of the paper to make our design choice more clear.


==> revision_files/reviewer3.tex <==
\section{Reviewer \#3}

\textbf{R3O1}:  One simple idea that comes to mind is to train a model per location and tune its seasonality. For example, NimbusML and exponential smoothing allow to set seasonality. In this way, the model would be location-aware and could still capture the daily/weekly pattern in Figure 1. Please clarify why this approach is insufficient and ideally evaluate its accuracy and overhead in experiments

\textbf{Response}: If we train a model for each location, we are unable to model the correlations among the sensors’ time series, which have already been shown in multiple recent studies \cite{dcrnn,agcrn,graphwavenet,stfgnn} to play a profound impact on the overall accuracy in the context of traffic time series forecasting. 

\hspace{0.4cm}To evaluate the accuracy of such ``per location'' models, we consider two variants. First, we train a distinct \texttt{Transformer}~\cite{attention_all_you_need} per location/sensor. Second, as suggested by the reviewer, we use Holt-Winters Exponential Smoothing \texttt{HWES} that is able to capture both a trend and a seasonal variation per location/sensor. % and our proposed spatially-aware enhanced version of attention \texttt{S-ATT}. We would like to note that for attention based methods methods, i.e. \texttt{Naive} and \texttt{S-ATT}, we have removed the component which models correlations among the sensors such that the results are comparable with \texttt{HWES}. 
%
The results are shown in Table \ref{table:naive} in the revision report, where \texttt{ST-WA} significantly outperforms the two ``per location'' models, which emphasize the importance of entity correlation modeling as well as location specific and time-varying model parameters. We can observe that \texttt{ST-WA} sometimes has a higher runtime when compared with some of the ``per location'' models. To strike a balance between efficiency and accuracy, we can use a modified version of the proposed Window Attention $\texttt{W-Att}$ where proxies are used but entity correlation modeling is removed. We see that $\texttt{W-Att}$ achieves better accuracy when compared with \texttt{HWES} and \texttt{Transformer} while being the fastest. 


%
%First we can observe that 
%\texttt{HWES} achieves impressive results, but it fall short when compared with the \texttt{Naive} approach. Next, when comparing the naive approach with the enhanced version of attention \texttt{ST-ATT} we can observe a significant performance improvement, which better motivates our design choices. Furthermore, if we look at the runtime which is presented in minutes, as there are no epochs for  \texttt{HWES} we can observe that \texttt{ST-ATT} is the fastest. This is because the \texttt{Naive} method suffer from high parameter space, and while \texttt{HWES} is fast it needs to be fitted after each forecast which incurs additional overhead. Finally, we observe that \texttt{ST-ATT} significantly outperforms \texttt{S-ATT} in terms of accuracy, but is slower as it needs to model entity correlations. 




\vspace{2em}
\textbf{R3O2}: Please clarify in introduction why is adding spatial and temporal information is a challenging problem. It seams easy to me as described above. These are just two additional features.

\textbf{Response}: We would like to clarify that we do not mean spatio-temporal features but spatio-temporal aware model parameters. We aim to learn distinct model parameters for different sensors (i.e., spatial aware) and during different time periods (i.e., temporal aware), thus being able to distinguish the distinct patterns from different sensors during different time periods. Most existing models are spatio-temporal agnostic, because they use the same model parameters for all sensors during all time periods. 

In addition, our approach is purely data driven, which avoids using additional location and time specific features, such as coordinates of sensor locations and prior knowledge on peak vs. offpeak hours. Except for the time series data itself, we do not require any additional information. 

We have revised the introduction as suggested to make this more clear.  

\vspace{2em}
\textbf{R3O3}: Please formulate the proposed approach as algorithms in Section 4 in addition to descriptions and complexity analysis.

\textbf{Response}:  We have formulated both our proposals Spatio-Temporal Aware Modeling and Window Attention as algorithms and include the corresponding pseudo code in Section III as suggested.



\vspace{2em}
\textbf{R3O4}: The paper is heavy on notation. Please add a table of notations to Section 3.

\textbf{Response}: We have added a table of notation in the beginning of Section III as suggested.


\vspace{2em}
\textbf{R3O5}: The code is on google drive and requires access permissions. Asking for permissions would reveal my identity. Please move the code to GitHub.

\textbf{Response}:  The code is now publicly available on GitHub at https://github.com/razvanc92/ST-WA.

